Disjointness through the Lens of Vapnik-Chervonenkis Dimension: Sparsity and Beyond

The disjointness problem - where Alice and Bob are given two subsets of $\{1, \dots, n\}$ and they have to check if their sets intersect - is a central problem in the world of communication complexity. While both deterministic and randomized communication complexities for this problem are known to be $\Theta(n)$, it is also known that if the sets are assumed to be drawn from some restricted set systems then the communication complexity can be much lower. In this work, we explore how communication complexity measures change with respect to the complexity of the underlying set system. The complexity measure for the set system that we use in this work is the Vapnik-Chervonenkis (VC) dimension. More precisely, on any set system with VC dimension bounded by $d$, we analyze how large can the deterministic and randomized communication complexities be, as a function of $d$ and $n$. In this paper, we construct two natural set systems of VC dimension $d$, motivated from geometry. Using these set systems we show that the deterministic and randomized communication complexity can be $\widetilde{\Theta}\left(d\log \left( n/d \right)\right)$ for set systems of VC dimension $d$ and this matches the deterministic upper bound for all set systems of VC dimension $d$. We also study the deterministic and randomized communication complexities of the set intersection problem when sets belong to a set system of bounded VC dimension. We show that there exists set systems of VC dimension $d$ such that both deterministic and randomized (one-way and multi-round) complexity for the set intersection problem can be as high as $\Theta\left( d\log \left( n/d \right) \right)$, and this is tight among all set systems of VC dimension $d$.

==> copy.tex <==
\section{Lower bound result for \vcdisj{n}{d}}\label{sec:vclower}

\begin{lem}\label{lem:disj}
$R_\delta(\mbox{\ddisj{n}{k}})=\Omega(nk)$.
\end{lem}

\begin{lem}\label{lem:subset}
$R_\delta(\mbox{\dsub{n}{k}})=\Omega(nk)$.
\end{lem}
\begin{proof}
The claim follows from  Lemma~\ref{lem:disj} along with the fact that $S \subseteq T$ if and only if $S \cap \overline{T}=\emptyset$. 

\end{proof}

\begin{lem}\label{lem:div}
$R_\delta(\mbox{\ddivs{n}{k}})=\Omega\left(\frac{kn}{\log n}\right)$
\end{lem}
\begin{proof}
Let by contradiction, assume that there exists a $\delta$-error randomized protocol $\cP$ that solves \ddivs{n}{k} with communication cost $o\left(\frac{k n}{\log n}\right)$. Now, we give a $\delta$-error protocol $\cP'$ that solves \dsub{t}{k} with communication cost $o\left(kt\right)$, where $t=cn/\log n$ for some suitable constant $c$. 
\paragraph*{Protocol $\cP'$ for \dsub{t}{k}} 
\begin{itemize}
\item  Let $A=({\bf a}_1,\ldots, {\bf a}_k) \in \left[\{0,1\}^{t} \right]^k$ and $B=({\bf b}_1,\ldots, {\bf b}_k) \in \left[\{0,1\}^{t} \right]^k$ be the inputs of Alice and Bob for \dsub{t}{k}. Both Alice and Bob privately determine first $t=cn/\log n$ prime numbers $p_1,\ldots,p_t$ with out any communication. Note that we can set $c$ such that
 $\prod_{i=1}^{t}p_i \leq 2^{n}$.
 \item Let $\Phi:\{0,1\}^t \rightarrow \{0,1\}^n$ be the function such that $\phi({\bf x})$ is the bit representation of $\prod_{x_i=1}p_i$. Alice finds $A'=(\phi({\bf a}_1),\ldots,\phi({\bf a}_k))$ and Bob finds $B'=(\phi({\bf b}_1),\ldots,\phi({\bf b}_k))$ privately with out any communication.  
 \item Then Alice and Bob solve \ddivs{n}{k} on inputs $A'$ and $B'$; and report $\mbox{\dsub{t}{k}}(A,B)=1$ if and only if $\mbox{\ddivs{n}{k}}(A',B')=1$.
\end{itemize}
The correctness of $\cP'$ follows from the following argument.

\begin{eqnarray*}
&&\mbox{\dsub{t}{k}}(A,B)=1\\
&\Leftrightarrow& ~\exists~j \in [k]~\mbox{ such that ${\bf a_j}$ is a subset of}~ {\bf b_j} \\
&\Leftrightarrow& ~\exists~j \in [k]~\mbox{ such that $\phi({\bf a_j})$ divides}~ \phi({\bf b_j})\\
&\Leftrightarrow& \mbox{\ddivs{n}{k}}(A',B')=1.
\end{eqnarray*} 
Note that the existence of $\cP'$ for $\mbox{\dsub{t}{k}}$, with communication cost $o\left(\frac{kn}{\log n}\right)=o(kt)$, contradicts Lemma~\ref{lem:subset}. Hence, we are done with the proof.
\end{proof}
\subsection{Proof of Theorem~\ref{theo:main}}
Consider the following set system $\cS=(\cG,\cL)$, which will be needed for our proof of Theorem~\ref{theo:main}.
\paragraph*{The ground set $\cG$}
Let $G_{(0,0)} =\{(x,y)\in \Z^2:0 \leq x,y \leq n-1\}$, the grid of size $n \times n$ centered at origin. For any $p, q \in \Z$, the grid having origin at $(p,q)$ is denoted and defined as $G_{(p,q)}=\{(i+p,j+q) : (i,j) \in G \}$. For $d \in \N$, consider $G_{(p_1,q_1)}, \ldots, G_{(p_{d},q_{d})}$ satisfying the following property.

{\sc Prop:} For any $i \neq j\in [d]$, if $L_1~(L_2)$ be a line of non-negative slope that passes through two points of $G_{(p_i,q_i)}~(G_{(p_j,q_j)})$, then $L_1$ and $L_2$ does not intersect at any point in $\bigcup_{\ell=1}^{d} G_{(p_\ell,q_\ell)}$. 

Observe that $G_{(p_1,q_1)}, \ldots, G_{(p_{d},q_{d})}$ exist satisfying {\sc Prop}. See Figure~\ref{} for an illustration. We take the ground set as
$$\cG = \bigcup_{\ell=1}^{d} G_{(p_\ell,q_\ell)}.$$
Note that with out loss of generality, we can assume that $(p_1,q_1)=(0,0)$.
\paragraph*{The set of ranges $\cL$}
$\cL$ contains two types of subsets of $\cG$, that is, $\cL_1$ and $\cL_2$ that are generated by the following ways.
\begin{itemize}
\item Take any $d$ lines $L_1,\ldots,L_d$ of non negative slope such that $L_i$ passes through $(p_i,q_i)$ and (at least) another point in $G_{(p_i,q_i)}$. Note that  $L_i$ does not intersect with any point in $\cG \setminus G_{(p_i,q_i)}$. The set $A=\bigcup_{i=1}^d (L_i \cap G_{(p_i,q_i)})$ is in $\cL_1$, and we say $A$ is generated by the lines $L_1,\ldots,L_d$.
\item Take any $d$ vertical lines $L'_1,\ldots,L'_d$ such that $L_i$ intersects with some points in $G_{(p_i,q_i)}$. Note that  $L_i$ does not intersect with any point in $\cG \setminus G_{(p_i,q_i)}$. The set $B=\bigcup_{i=1}^d (L_i \cap G_{(p_i,q_i)})$ is in $\cL_2,$ and we say $B$ is generated by the lines $L'_1,\ldots,L'_d$. 
\end{itemize} 

\begin{obs}
The {\sc Vc-Dimension} of $\cS$ is $2d$.
\end{obs}



\begin{obs}\label{obs:inter1}
Let $A \in \cL_1$ and $B \in \cL_2$ such that $A$ is generated by lines $L_1,\ldots,L_d$ and $A$ is generated by lines $L'_1,\ldots,L'_d$. Then $A$ and $B$ intersect if and only if there exists $i \in [d]$ such that $L_i$ and $L_i'$ intersect at a point in $G_{(p_i,q_i)}$.  
\end{obs}

\begin{obs}\label{obs:inter}
Let $A \in \cL_1$ and $B \in \cL_2$ such that $A$ is generated by lines $L_1,\ldots,L_d$ and $A$ is generated by lines $L'_1,\ldots,L'_d$. Also let $\size{A \cap B}=d$. Then for each $i \in [d]$, $L_i$ and $L_i'$ intersect at a point in $G_{(p_i,q_i)}$. Moreover, $A$ ($B$) can be determined if we know $B$ ($A$) and $A \cap B$.
\end{obs}

Now, we are ready to prove Theorem~\ref{theo:main} and Theorem~\ref{theo:main1}.
\begin{proof}[Proof of Theorem~\ref{theo:main}]
Let by contradiction, assume that there exists a $\delta$-error randomized protocol $\cP$ that solves \vcdisj{n}{2d} on the set system $\cS=(\cG,\cL)$ with communication cost $o\left( \frac{d \log n}{\log \log n}\right)$. Now, we give a $\delta$-error protocol $\cP'$ that solves \ddivs{\log n}{d} with communication cost $o\left( \frac{d \log n}{\log \log n}\right)$.
\paragraph*{Protocol $\cP'$ for \ddivs{\log n}{d}}
\begin{itemize}
\item Let $A=({\bf a}_1,\ldots,{\bf a}_{\log n}) \in \left[\{0,1\}^{\log n}\right]^{d}$ and $B ({\bf a}_1,\ldots,{\bf a}_{\log n})\in \left[ \{0,1\}^{\log n}\right]^{d}$ be the inputs of Alice and Bob for \ddivs{\log n}{d}. 
\item For each $i \in [d]$, let $L_i$ and $L_i'$ be the lines having equation $y-q_i=\frac{\val{{\bf a}_i}-1}{\val{{\bf a}_i}}(x-p_i)$ and $x-p_i=\val{b_i}$. Alice finds $A' \in \cL$ that is generated by the lines $L_1,\ldots,L_d$, and Bob finds $B' \in \cL$ which is generated by the lines $L'_1,\ldots,L'_d$.
\item Then Alice and Bob solve \vcdisj{n}{2d} on inputs $A'$ and $B'$, and report $\mbox{\ddivs{\log n}{d}}(A,B)=1$ if and only if 
$\mbox{\vcdisj{n}{2d}}(A',B')=1$.
\end{itemize}
The correctness of the protocol follows from the following argument..

\begin{eqnarray*}
&&\mbox{\vcdisj{n}{2d}}(A',B')=1\\
&\Leftrightarrow&  A' \cap B' =\emptyset \\
&\Leftrightarrow&  \mbox{ $\exists i \in [d]$ such that the lines $L_i:y-q_i=\frac{\val{{\bf a}_i}-1}{\val{{\bf a}_i}}(x-p_i)$ and $L_i':x-p_i=\val{\bf{b_i}}$}\\
&& \mbox{intersect at a point in $G_{(p_i,q_i)}$}~~(\mbox{By Observation~\ref{obs:inter}})\\
&\Leftrightarrow&  \mbox{ $\exists i \in [d]$ such that the lines $y=\frac{\val{{\bf a}_i}-1}{\val{{\bf a}_i}}x$ and $ x=\val{{\bf b}_i}$ intersect at a point in $G_{(0,0)}$}\\
&\Leftrightarrow& \mbox{ $\exists i \in [d]$ such that $\val{{\bf a}_i}$ divides $\val{{\bf b_i}}$}\\
&\Leftrightarrow&  \mbox{\ddivs{\log n}{d}}(A,B)=1\\
\end{eqnarray*} 

As the existence of $\cP'$ for \ddivs{\log n}{d}, with communication cost $o\left( \frac{d \log n}{\log \log n}\right)$, contradicts Lemma~\ref{lem:div}. Hence, we are done with the proof.

\end{proof}

\begin{proof}[Proof of Theorem~\ref{theo:main1}]
First, consider the following problem where the objective of Alice and Bob learn each other's set.

\defproblem{\vclearn{n}{d}}{Alice and Bob get two sets $A$ and $B$, respectively, from  ${\cal S}=({\cal G},{\cal L})$ with a promise that $A \cap B =d$.}{Alice learns $B$ and Bob learns $A$.}

Observe that $R({\mbox{\vclearn{n}{d}}})=\Omega(d \log n)$ as there are $\Omega(n^d)$ many candidate sets for the input of Alice as well as Bob. We proof the desired lower bound by reducing \vclearn{n}{d} to a special case of \vcint{n}{d} when the underlying set system is ${\cal S}=({\cal G},{\cal L})$ and it is promised that $\size{A \cap B}=d$. Let by contradiction consider a protocol ${\cal P}$ that solves \vcint{n}{d} on ${\cal S}$ and uses $o(d \log n)$ bits of communication. To solve \vclearn{n}{d}, Alice and Bob first run protocol {\cal P} and finds $A \cap B$. Then Alice (Bob) can determine $B$ ($A$) by combining $A$ ($B$) along with $A \cap B$, which is possible by Observation~\ref{obs:inter1}, with any communication with Bob (Alice). Now, we have a protocol ${\cal P}'$ that solves \vclearn{n}{d} with $o(d \log n)$ bits of communication, which is not possible.

\end{proof}
\section{Proof of Theorem~\ref{theo:main-oneway}}
Consider the following set system ${\cal Q}=(X,{\cal R})$ that will be required in our lower bound proof of Theorem~\ref{theo:main-oneway}.

\paragraph*{The set system ${\cal Q}$:}
Let $I_o=\{0,\ldots,n+1\}$, that is the interval of length $n+1$ that starts at origin and ends at $n+1$. Let $I_p$ be the interval of length $n+1$ that starts at $p \in \Z$ and ends at $p+n+1$. For $d \in \N$, consider $d$ pairwise disjoint sets $I_{p_1},\ldots,I_{p_d}$. The ground set $X=\bigcup\limits_{i=1}^d I_{p_i}$. ${\cal R}$ contains two types of sets ${\cal R}_0$ and ${\cal R}_{n+1}$, where
\begin{itemize}
\item Take any $d$ intervals $R_1, \ldots,R_d$ of length at most $n+1$ such that $R_i$ starts at $p_i$ for each $i \in [d]$. Note that $R_i$ does not intersect with any $X \setminus I_{p_i}$. The set $A=\bigcup\limits_{i=1}^d R_i$ is in ${\cal R}_0$. We say that $A$ is generated by $R_1,\ldots,R_d$.
\item Take any $d$ intervals $R'_1, \ldots,R'_d$ of length at most $n+1$ such that $R_i$ ends at $p_i+n+1$ for each $i \in [d]$. Note that $R'_i$ does not intersect with any $X \setminus I_{p_i}$. The set $B=\bigcup\limits_{i=1}^d R'_i$  is in ${\cal R}_{n+1}$. We say that $A$ is generated by $R'_1,\ldots,R'_d$.
\end{itemize}
\begin{obs}
The VC-dimension of ${\cal Q}$ is $d$.
\end{obs}
\begin{obs}{obs:interval-oneway}
Let $A \in {\cal R}_0$ and $B \in {\cal R}_{n+1}$ such that $A$ is generated by $R_1,\ldots,R_d$ and $B$ is generated by $R'_1,\ldots,R'_d$. Then $A$ and $B$ intersects if and only if there exists an $i \in [d]$ such  that $R_i$ intersects $R'_i$ at a point in $I_{p_i}$. 
\end{obs}
Now, we are ready to prove Theorem~\ref{theo:main-oneway}.
\begin{proof}[Proof of Theorem~\ref{theo:main-oneway}]
We show the desired lower bound for \vcdisj{d}{n} by reducing from a problem {\sc Augmented Indexing}, over $d \log n$ bits, defined as follows. In Augmented Indexing, Alice gets a string $\{\bf x\} \in \{0,1\}^{d \log n}$ and Bob gets an index $j \in [d \log n]$ and all $x_{j'}$ for $j'<j$. The objective of the Bob is to receive a single message from Bob and output $x_j$. The one-way communication complexity of  {\sc Augmented Indexing} is $\Omega(d \log n)$~\cite{}.

 Let ${\cal P}$ be an one-way protocol that solves \vcdisj{d}{n}, on the set system $Q$, with $o(d \log n)$ bits of communication. Now, we consider the following protocol ${\cal P}'$ for {\sc Augmented Indexing}.
 
 \paragraph*{Protocol ${\cal P}'$ for {\sc Augmented Indexing} problem}
 \begin{itemize}
 \item Let ${\bf x} \in \{0,1\}^{d \log n}$ be the input of Alice; $j \in [d \log n]$ and $x_{j'}$ for each $j' < j$ be the input of Bob.
 \item Alice will form $d$ strings ${\bf a}_1,\ldots, {\bf a}_{d} \in \{0,1\}^{\log n}$ by truncating the 
 string ${\bf x}$ in to $d$ parts such that ${\bf a}_i=x_{(i-1)\log n+1}\ldots x_{i \log n} $, where $i \in [d]$. Bob first form a string ${\bf y} \in {0,1}^n$, where $y_{j'}=x_{j'}$ for each $j' < j$, $y_j=0$, and $y_{j'}=0$ for each $j'>j$. Then Bob finds ${\bf b}_1,\ldots, {\bf b}_{d} \in \{0,1\}^{\log n}$ by truncating the 
 string ${\bf y}$ in to $d$ parts such that ${\bf b}_i=y_{(i-1)\log n+1}\ldots y_{ i \log n} $, where $i \in [d]$.
 \item For each $i \in [d]$, let $R_i$ and $R_i'$ be the intervals that starts at $p_i$ and ends at $p_i+n+1$, respectively, where $R_i=\{p_i,\ldots,n+p_i-\val{{\bf a}_i}\}$ and $R_i=\{n+1-\val{{\bf b }_i},\ldots,p_i+n+1\}$. Alice finds the set $A \in {\cal R}_0$ that is generated by $R_1,\ldots,R_d$ and Bob finds the set $B \in {\cal R}_{n+1}$ that is generated by $R'_1,\ldots,R'_d$.
 \item Alice and Bob solves \vcdisj{n}{d} on inputs $A$ and $B$, and report $1$ as the output of {\sc Augmented Indexing} problem if and only if \vcdisj{n}{d}($A,B$)$=1$.
 \end{itemize}
Now, the correctness of protocol ${\cal P}'$ follows from the Observation.  Let $i^* \in [d]$ such that $j \in \{(i^*-1) \log n+1,i^* \log n\}$.
\begin{obs}\label{obs:correct}
\begin{itemize}
\item[(i)] $R_i \cap R'_i =\emptyset$ for all $i \neq i^*$.
\item[(ii)] $R_{i^*} \cap R'_{i^*} =\emptyset$ if and only if $\val{{\bf b}_{i^*}} \leq  \val{{\bf b}_{i^*}}$.
\item[(iii)]  $\val{{\bf b}_{i^*}} \leq  \val{{\bf b}_{i^*}}$ if and only if $x_j=0$.
\end{itemize}
\end{obs}
For the sake of completeness of correctness proof of protocol ${\cal P}'$, 
 \begin{eqnarray*}
&& \mbox{\vcdisj{n}{d}}(A,B) =0 \\
 & \Leftrightarrow& \mbox{There exists an $i \in [d]$} such that R_{i} \cap R'_{i}\neq \emptyset ~~(\mbox{By Observation~\ref{obs:inter:interval-oneway}})\\
 & \Leftrightarrow& R_{i*} \cap R'_{i^*}=\emptyset~~(\mbox{By Observation~\ref{obs:correct}(i)}) \\
 & \Leftrightarrow&  x_j=0 ~~(\mbox{By Observation~\ref{obs:correct}(i) and (ii)})
 \end{eqnarray*}
The one-way communication complexity of protocol ${\cal P}'$ is the same as that of ${\cal P}$, that is, $o(d \log n)$. However, this is impossible as the one-way communication complexity of {\sc Augmented Indexing }, over $d \log n$ bits, is $\Omega(d \log n)$ bits.
\end{proof}

==> direct-sum.tex <==
\section{Lower bound for existence of a pair of disjoint set (\ddisj_{n}{k})}
\label{sec:direct}
\begin{lem}
$R(\mbox{\ddisj_{n}{k}})=\Omega(nk)$.
\end{lem}
\begin{proof}

\end{proof}

==> upperbounds.tex <==
\remove{\section{Upper bounds}
\subsection{Upperbound for \divs{n}}
In this section, we discuss a randomized protocol for \divs{n} with communication cost $O\left( \frac{n}{\log n} \log \log n\right)$.
\begin{algorithm}[H]
%\scriptsize
\caption{Protocol for \divs{n}}
\label{algo_div}
\KwIn{Alice has ${\bf a} \in \{0,1\}^n$ and Bob has ${\bf b} \in \{0,1\}^n$.}
\KwOut{$1$ if ${\bf a}$ divides ${\bf b}$, Otherwise $0$.}
%\LinesNumbered
\Begin
	{
	
	 Alice and Bob factorize $\val({\bf a})$ and ${\val{{\bf b}}$, respectively. Let $P_a$ and $P_b$ be the prime factors.
	
	For each $i \in [\alpha \log n]$ and $r,s \in [\beta K]$, initiate an $\ell_0$ sampler $L^i_{r,s}$.
	
	\For{ (each $(u,v)$ in the stream)}
	{
	Irrespective of $(u,v)$ being inserted or deleted, give the respective input to the $\ell_0$-samplers $L_{h_i(u),h_i(v)}^i$ for each $i \in [\alpha \log n]$.
	}
	
	For each $i \in [\alpha \log n]$, construct a 
subgraph $H_i$  by taking the outputs of all the $\ell_0$-samplers corresponding to the hash function $h_i$.

Construct $H =H_1 \cup \cdots \cup H_{\alpha \log n}$.

Run the classical {\sc FPT} algorithm for \cvd on the subgraph $H$ and solution size bound $k$~\cite{saketbook15}.

\If{($H$ has a solution $S$ of size at most $k$)}
{Report $S$ as the solution to $G$.}
\Else{
Report {\sc Null}}

}
\end{algorithm}}
